Random Access with Physical-layer Network Coding

Leveraging recent progress in physical-layer network coding we propose a new approach to random access: When packets collide, it is possible to recover a linear combination of the packets at the receiver. Over many rounds of transmission, the receiver can thus obtain many linear combinations and eventually recover all original packets. This is by contrast to slotted ALOHA where packet collisions lead to complete erasures. The throughput of the proposed strategy is derived and shown to be significantly superior to the best known strategies, including multipacket reception.

==> analysis.tex <==





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Slotted ALOHA} \label{sec:aloha}
If users transmit at rate
\begin{equation}
 R = \frac{1}{2}\log(1+a^{-1}P),
\end{equation}
the receiver is only able to decode if there is a single active user.

\begin{theorem}
Slotted ALOHA achieves throughput
\begin{equation}
 T = Ka(1-a)^{K-1}\frac{1}{2}\log\left(1+a^{-1}P\right).
\end{equation}
\end{theorem}
\begin{proof}
todo.
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Rate adaption with multipacket reception} \label{sec:superposition}
The first strategy we consider is the adaptive rate approach as used in for instance~\cite{medard2004capacity}.

Under this strategy all users transmit at rate
\begin{equation}
 R=\frac{1}{2K}\log\left[1+Ka^{-1}P\right].
\end{equation}
This ensures that the decoder can always decode. The throughput equals
\begin{equation}
 T = K a R = \frac{a}{2}\log\left[1+Ka^{-1}P\right].
\end{equation}
Only a single block is used, \ie $N=1$.
\begin{theorem}[\cite{medard2004capacity}, \cite{minero2012random}]
A rate
\begin{equation}
 T =  \frac{a}{2}\log\left[1+Ka^{-1}P\right]
\end{equation}
is achievable by using a layered strategy.
\end{theorem}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Ignoring CSI strategy} \label{sec:ignore}
If we ignore CSI we have an ordinary fading channel for which capacity is known~\cite{hanly1998multiaccess}. In this case the users can not use power $a^{-1}P$ in active blocks, but are restricted to using average power $P$ in all blocks. For two users we have
\begin{equation}
 T = a(1-a)\log[1 + P] + \frac{a^2}{2}\log[1 + 2P].
\end{equation}
The $K$ user case is treated next.
\begin{theorem}
A throughput
\begin{equation}
 T = \sum_{i=1}^K \binom{K}{i}a^i(1-a)^{K-i}\frac{1}{2}\log\left(1+i P\right).
\end{equation}
is achievable by ignoring CSI.
\end{theorem}
\begin{IEEEproof}
The constraint on the sum rate of all users is really the bottleneck.
\end{IEEEproof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Other strategies}
Other strategies have been proposed in the literature. In~\cite{minero2012random}, for instance, a superposition strategy is proposed in which different layers are used. However, as oberved in~\cite{minero2012random}, on the AWGN channel it is optimal to use a single layer. 

% As commented on in~\cite{minero2012random} the best known strategy for AWGN channels is in fact to not use layers, but do either collision or rate adaption strategy.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Upper bound} \label{sec:upper}
We construct an upper bound by considering the case that users have complete knowledge of the state of all users.  A well known result, \cf~\cite{elgamalkim}, is that in this case the sum rate is upper bounded as
\begin{equation} \label{eq:upperstart}
 T \leq \EE\left[\frac{1}{2}\log\left(1+\sum_{i=1}^K S_i a^{-1} P\right)\right], 
\end{equation}
where the expectation is over the user states. For two users the bound reduces to
\begin{equation}
 T \leq a(1-a)\log\left[1+a^{-1}P\right] + \frac{a^2}{2}\log\left(1+2a^{-1}P\right).
\end{equation}
The general case follows readily by observing the number of active users is binomially distributed and is given in the next theorem.
\begin{theorem}
If throughput $T$ is achievable, then
\begin{equation}
 T \leq \sum_{i=1}^K \binom{K}{i}a^i(1-a)^{K-i}\frac{1}{2}\log\left(1+ia^{-1}P\right).
\end{equation}
\end{theorem}
% \begin{IEEEproof}
%  Starting from~\eqref{eq:upperstart} we have
% \end{IEEEproof}








%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Physical-layer network coding strategy} \label{sec:strategy}
% Moved to other section.

